Multi-wavelength observations of the black widow pulsar 2FGL J2339.6-0532 with OISTER and Suzaku

Multi-wavelength observations of the black-widow binary system 2FGL J2339.6-0532 are reported. The Fermi gamma-ray source 2FGL J2339.6-0532 was recently categorized as a black widow in which a recycled millisecond pulsar (MSP) is evaporating up the companion star with its powerful pulsar wind. Our optical observations show clear sinusoidal light curves due to the asymmetric temperature distribution of the companion star. Assuming a simple geometry, we constrained the range of the inclination angle of the binary system to 52$^{\circ}$ < i < 59$^{\circ}$, which enables us to discuss the interaction between the pulsar wind and the companion in detail. The X-ray spectrum consists of two components: a soft, steady component that seems to originate from the surface of the MSP, and a hard variable component from the wind-termination shock near the companion star. The measured X-ray luminosity is comparable to the bolometric luminosity of the companion, meaning that the heating efficiency is less than 0.5. In the companion orbit, 10$^{11}$ cm from the pulsar, the pulsar wind is already in particle dominant-stage, with a magnetization parameter of $\sigma$ < 0.1. In addition, we precisely investigated the time variations of the X-ray periodograms and detected a weakening of orbital modulation. The observed phenomenon may be related to an unstable pulsar-wind activity or a weak mass accretion, both of which can result in the temporal extinction of radio-pulse.

==> table_5.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{deluxetable}{lcc}
\tabletypesize{\scriptsize}
\tablecolumns{3}
\tablecaption{Obtained parameters of the binary system from the phase-resolved SED\label{SEDfit_results}}
\tablewidth{0pt}
\tablehead{
 \colhead{Data set}& 
 \colhead{Optical+IR\tablenotemark{a}}&
 \colhead{Optical\tablenotemark{a}}
}
\startdata
 Orbital radius ($R_{\rm orb}$)\tablenotemark{b}&
 $1.08 \pm 0.02 \quad \times 10^{11}$ cm&
 $1.18 \pm 0.02 \quad \times 10^{11}$ cm\\
 Companion radius ($r_{\rm comp}$) &
 $1.26 \pm 0.02 \quad \times 10^{10} \; d_{\rm 1.1}$ cm\tablenotemark{c}&
 $1.53 \pm 0.02 \quad \times 10^{10} \; d_{\rm 1.1}$ cm\tablenotemark{c}\\
 Companion Temperature ($T_{\rm cool}$)&
 $3170 \pm  70  \quad$ K&
 $2740 \pm 120  \quad$ K\\
 Heating Efficiency ($f$)\tablenotemark{d}&
 $1.42 \pm 0.05$&
 $1.16 \pm 0.04$\\
 Inclination angle ($i$)&
 $59.\degr0 \pm 1.\degr5$&
 $52.\degr1 \pm 1.\degr0$\\
 Bolometric Luminosity\tablenotemark{e}&
 $1.09 \pm 0.17\quad \times10^{32}\; d_{\rm 1.1}^2$ erg s$^{-1}$&
 $1.12 \pm 0.16\quad \times10^{32}\; d_{\rm 1.1}^2$ erg s$^{-1}$\\
 $\chi^2$ & 1392.6& 637.6\\
\enddata
\tablecomments{Errors are with 1 $\sigma$ confidence level.}  
\tablenotetext{a}{``Optical'' and ``IR'' correspond to [B, V, R, I, g']
 data-set and  [J, H, Ks] data-set, respectively.}  
\tablenotetext{b}{$R_{\rm orb}$ are calculated based on radial velocity
 of the companion star reported by \cite{2011ApJ...743L..26R}.}  
\tablenotetext{c}{$d_{\rm 1.1}$ is the distance in unit of 1.1 kpc.}  
\tablenotetext{d}{Assuming an isotropic pulsar wind with a luminosity of
 $2.3\times10^{34}$ erg s$^{-1}$ based on \cite{2014AAS...22314007R}.}
\tablenotetext{e}{Bolometric luminosity of the companion's heated hemisphere.}
\end{deluxetable}
%\endinput




\begin{deluxetable}{lcc}
\tabletypesize{\scriptsize}
\tablecolumns{3}
%\rotate
\tablecaption{Results of model fitting of the averaged X-ray spectra\label{spec_results}
}
\tablewidth{0pt}
\tablehead{
 \colhead{Model} & 
 \colhead{wabs*(bbody + power-law)}&
 \colhead{wabs*power-law}
}
\startdata
$N_{\rm H}$ ($10^{21}$ cm$^{-2}$) &
$ < 1.2$ (0) &  $ < 0.13$ (0) \\
Blackbody Temperature (keV)&
 $0.15 \pm 0.06$  & \nodata \\
Blackbody Radius (km)\tablenotemark{\dagger} &
 $0.28^{+0.93}_{-0.16}\quad$ & \nodata\\
Power-law Photon Index&
 $1.14^{+0.14}_{-0.15}$ & $1.32\pm0.08$ \\ 
Power-law Flux$_{\rm 0.5-10keV}$ ($10^{-13}$ erg cm$^{-2}$ s$^{-1}$)&
 $2.50 \pm 0.16$ & $2.50 \pm 0.15$\\
Total flux$_{\rm 0.5-10keV}$ ($10^{-13}$erg cm$^{-2}$ s$^{-1}$)&
 $2.67^{+0.01}_{-1.25}$&  $2.46^{+0.04}_{-0.73}$\\
 $\chi^2$ (dof)&
 51.82 (51) & 67.71(53)\\
\enddata
%% Text for table notes should follow after the \enddata but before
%% the \end{deluxetable}. Make sure there is at least one \tablenotemark
%% in the table for each \tablenotetext.
\tablecomments{Errors are with 90 \% confidence level.}
\tablenotetext{\dagger}{Blackbody radius assuming a distance of 1.1 kpc.}
\end{deluxetable}
\endinput


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% End of file `table.tex'.

